Measurements of four-lepton production in $pp$ collisions at $\sqrt{s}=$ 8 TeV with the ATLAS detector

The four-lepton ($4\ell$, $\ell = e, \mu$) production cross section is measured in the mass range from 80 to 1000 GeV using 20.3 fb$^{-1}$ of data in $pp$ collisions at $\sqrt{s}=8$ TeV collected with the ATLAS detector at the LHC. The $4\ell$ events are produced in the decays of resonant $Z$ and Higgs bosons and the non-resonant $ZZ$ continuum originating from $q\bar q$, $gg$, and $qg$ initial states. A total of 476 signal candidate events are observed with a background expectation of $26.2 \pm 3.6$ events, enabling the measurement of the integrated cross section and the differential cross section as a function of the invariant mass and transverse momentum of the four-lepton system. In the mass range above $180$ GeV, assuming the theoretical constraint on the $q\bar q$ production cross section calculated with perturbative NNLO QCD and NLO electroweak corrections, the signal strength of the gluon-fusion component relative to its leading-order prediction is determined to be $\mu_{gg}=2.4 \pm 1.0 (stat.) \pm 0.5 (syst.)\pm 0.8 (theory)$.

==> Numbers.tex <==
\newcommand\AltMllCut{\ensuremath{ 4}}
\newcommand\MllCut{\ensuremath{ 5}}

\newcommand\LumiSevenTeV{\ensuremath{ 4.5\text{ fb}^{-1}}}
\newcommand\LumiEightTeV{\ensuremath{ 20.3\text{ fb}^{-1}}}
\newcommand\LumiUncertaintySevenTeV{\ensuremath{ 1.8\%}}
\newcommand\LumiUncertaintyEightTeV{\ensuremath{ 2.8\%}}

\newcommand\TotalZXsecTheorySevenTeV{\ensuremath{ 26.0 \pm 0.6\text{ nb}}}
\newcommand\TotalZXsecTheoryEightTeV{\ensuremath{ 30.3 \pm 0.8\text{ nb}}}
\newcommand\TotalZXsecObsSevenTeV{\ensuremath{ 27.3 \pm 0.3\text{ (syst)} \pm 0.5\text{ (lumi)}\text{ nb}}}
\newcommand\TotalZXsecObsEightTeV{\ensuremath{ 31.0 \pm 0.3\text{ (syst)} \pm 0.9\text{ (lumi)}\text{ nb}}}
\newcommand\ZmumuBR{\ensuremath{ \left( 3.366 \pm 0.007 \right)\%}}
\newcommand\ZmumuBkgSevenTeV{\ensuremath{ 3400 \pm 379}}
\newcommand\ZmumuBkgEightTeV{\ensuremath{ 19946 \pm 3976}}
\newcommand\ZmumuBkgQCDSevenTeV{\ensuremath{ 198 \pm 59}}
\newcommand\ZmumuBkgQCDEightTeV{\ensuremath{ 9905 \pm 2972}}
\newcommand\ZmumuBkgOtherSevenTeV{\ensuremath{ 3202 \pm 320}}
\newcommand\ZmumuBkgOtherEightTeV{\ensuremath{ 10041}}
\newcommand\AzmumuSevenTeV{\ensuremath{ \left( 41.4 \pm 0.6 \right)\%}}
\newcommand\AzmumuEightTeV{\ensuremath{ \left( 41.8 \pm 0.6 \right)\%}}
\newcommand\UZMuMSUpEightTeV{\ensuremath{ -0.006\%}}
\newcommand\UZMuMSDnEightTeV{\ensuremath{ 0.005\%}}
\newcommand\UZMuIDUpEightTeV{\ensuremath{ -0.003\%}}
\newcommand\UZMuIDDnEightTeV{\ensuremath{ 0.008\%}}
\newcommand\UZMuScaleUpEightTeV{\ensuremath{ 0.047\%}}
\newcommand\UZMuScaleDnEightTeV{\ensuremath{ -0.038\%}}
\newcommand\UZMuIdEffUpEightTeV{\ensuremath{ 0.654\%}}
\newcommand\UZMuIdEffDnEightTeV{\ensuremath{ -0.652\%}}
\newcommand\UZMuTrigUpEightTeV{\ensuremath{ 0.638\%}}
\newcommand\UZMuTrigDnEightTeV{\ensuremath{ -0.638\%}}
\newcommand\UZIsoIPUpEightTeV{\ensuremath{ 0.085\%}}
\newcommand\UZIsoIPDnEightTeV{\ensuremath{ -0.084\%}}

\newcommand\ZmumuObsSevenTeV{\ensuremath{ 1,725,523}}
\newcommand\ZmumuObsEightTeV{\ensuremath{ 8,868,653}}
\newcommand\ZmumuExpSevenTeV{\ensuremath{ 1,710,113}}
\newcommand\ZmumuExpEightTeV{\ensuremath{ 8,722,453}}

\newcommand\ObsEEEESevenTeV{\ensuremath{ 1}}
\newcommand\ObsEEMMSevenTeV{\ensuremath{ 7}}
\newcommand\ObsMMEESevenTeV{\ensuremath{ 5}}
\newcommand\ObsMMMMSevenTeV{\ensuremath{ 8}}
\newcommand\ObsAllSevenTeV{\ensuremath{ 21}}
\newcommand\ObsEEEEEightTeV{\ensuremath{ 85}}
\newcommand\ObsEEMMEightTeV{\ensuremath{ 136}}
\newcommand\ObsMMEEEightTeV{\ensuremath{ 99}}
\newcommand\ObsMMMMEightTeV{\ensuremath{ 156}}
\newcommand\ObsAllEightTeV{\ensuremath{ 476}}
\newcommand\ObsAllTotal{\ensuremath{ 172}}

\newcommand\ExpectedSigEEEEEightTeV{\ensuremath{  74.68 \pm 0.36 \pm 3.69}}
\newcommand\ExpectedSigEEMMEightTeV{\ensuremath{  94.96 \pm 0.48 \pm 2.24}}
\newcommand\ExpectedSigMMEEEightTeV{\ensuremath{  93.47 \pm 0.48 \pm 2.88}}
\newcommand\ExpectedSigMMMMEightTeV{\ensuremath{ 139.17 \pm 0.50 \pm 2.64}}
\newcommand\ExpectedSigAllEightTeV{\ensuremath{  402.28 \pm 0.92 \pm 9.17}}
\newcommand\ExpectedSigGGEEEEEightTeV{\ensuremath{  6.24 \pm 0.03 \pm 0.31}}
\newcommand\ExpectedSigGGEEMMEightTeV{\ensuremath{  8.26 \pm 0.03 \pm 0.20}}
\newcommand\ExpectedSigGGMMEEEightTeV{\ensuremath{  7.74 \pm 0.03 \pm 0.24}}
\newcommand\ExpectedSigGGMMMMEightTeV{\ensuremath{ 11.00 \pm 0.03 \pm 0.21}}
\newcommand\ExpectedSigGGAllEightTeV{\ensuremath{  33.25 \pm 0.06 \pm 0.76}}
\newcommand\ExpectedSigNNLOEEEEEightTeV{\ensuremath{  82.10 \pm 0.38 \pm 4.06}}
\newcommand\ExpectedSigNNLOEEMMEightTeV{\ensuremath{ 103.84 \pm 0.52 \pm 2.45}}
\newcommand\ExpectedSigNNLOMMEEEightTeV{\ensuremath{ 102.86 \pm 0.52 \pm 3.17}}
\newcommand\ExpectedSigNNLOMMMMEightTeV{\ensuremath{ 151.05 \pm 0.53 \pm 2.87}}
\newcommand\ExpectedSigNNLOAllEightTeV{\ensuremath{  439.86 \pm 0.98 \pm 10.02}}
\newcommand\ExpectedSigNonGGNNLOEEEEEightTeV{\ensuremath{  68.44 \pm 0.33 \pm 3.38}}
\newcommand\ExpectedSigNonGGNNLOEEMMEightTeV{\ensuremath{  86.70 \pm 0.45 \pm 2.05}}
\newcommand\ExpectedSigNonGGNNLOMMEEEightTeV{\ensuremath{  85.73 \pm 0.45 \pm 2.64}}
\newcommand\ExpectedSigNonGGNNLOMMMMEightTeV{\ensuremath{ 128.17 \pm 0.46 \pm 2.44}}
\newcommand\ExpectedSigNonGGNNLOAllEightTeV{\ensuremath{  369.03 \pm 0.85 \pm 8.41}}
\newcommand\ExpectedSigGGNNLOEEEEEightTeV{\ensuremath{ 13.66 \pm 0.05 \pm 0.67}}
\newcommand\ExpectedSigGGNNLOEEMMEightTeV{\ensuremath{ 17.14 \pm 0.07 \pm 0.41}}
\newcommand\ExpectedSigGGNNLOMMEEEightTeV{\ensuremath{ 17.13 \pm 0.07 \pm 0.53}}
\newcommand\ExpectedSigGGNNLOMMMMEightTeV{\ensuremath{ 22.89 \pm 0.07 \pm 0.43}}
\newcommand\ExpectedSigGGNNLOAllEightTeV{\ensuremath{  70.83 \pm 0.13 \pm 1.61}}

\newcommand\ExpectedSigAllTotal{\ensuremath{ 168.39}}

\newcommand\ExpGluonMCEEEESevenTeV{\ensuremath{ 0.004}}
\newcommand\ExpGluonMCEEMMSevenTeV{\ensuremath{ 0.005}}
\newcommand\ExpGluonMCMMEESevenTeV{\ensuremath{ 0.006}}
\newcommand\ExpGluonMCMMMMSevenTeV{\ensuremath{ 0.012}}
\newcommand\ExpGluonMCEEEEEightTeV{\ensuremath{ 0.021}}
\newcommand\ExpGluonMCEEMMEightTeV{\ensuremath{ 0.039}}
\newcommand\ExpGluonMCMMEEEightTeV{\ensuremath{ 0.034}}
\newcommand\ExpGluonMCMMMMEightTeV{\ensuremath{ 0.069}}
\newcommand\ExpTauMCEEEESevenTeV{\ensuremath{ 0.006}}
\newcommand\ExpTauMCEEMMSevenTeV{\ensuremath{ 0.019}}
\newcommand\ExpTauMCMMEESevenTeV{\ensuremath{ 0.009}}
\newcommand\ExpTauMCMMMMSevenTeV{\ensuremath{ 0.026}}
\newcommand\ExpTauMCEEEEEightTeV{\ensuremath{ 0.041}}
\newcommand\ExpTauMCEEMMEightTeV{\ensuremath{ 0.112}}
\newcommand\ExpTauMCMMEEEightTeV{\ensuremath{ 0.094}}
\newcommand\ExpTauMCMMMMEightTeV{\ensuremath{ 0.232}}
\newcommand\ExpDibosMCEEEESevenTeV{\ensuremath{ 0.010 \pm 0.002}}
\newcommand\ExpDibosMCEEMMSevenTeV{\ensuremath{ 0.024 \pm 0.002}}
\newcommand\ExpDibosMCMMEESevenTeV{\ensuremath{ 0.015 \pm 0.002}}
\newcommand\ExpDibosMCMMMMSevenTeV{\ensuremath{ 0.038 \pm 0.003}}
\newcommand\ExpDibosMCAllSevenTeV{\ensuremath{ 0.087 \pm 0.004}}
\newcommand\ExpDibosMCEEEEEightTeV{\ensuremath{ 0.064 \pm 0.009}}
\newcommand\ExpDibosMCEEMMEightTeV{\ensuremath{ 0.156 \pm 0.019}}
\newcommand\ExpDibosMCMMEEEightTeV{\ensuremath{ 0.132 \pm 0.017}}
\newcommand\ExpDibosMCMMMMEightTeV{\ensuremath{ 0.301 \pm 0.026}}
\newcommand\ExpDibosMCAllEightTeV{\ensuremath{ 0.653 \pm 0.038}}

\newcommand\ExpBkgMCEEEEEightTeV{\ensuremath{ 1.14 \pm 0.08 \pm 0.18}}
\newcommand\ExpBkgMCEEMMEightTeV{\ensuremath{ 1.55 \pm 0.09 \pm 0.26}}
\newcommand\ExpBkgMCMMEEEightTeV{\ensuremath{ 1.36 \pm 0.09 \pm 0.24}}
\newcommand\ExpBkgMCMMMMEightTeV{\ensuremath{ 1.91 \pm 0.10 \pm 0.34}}
\newcommand\ExpBkgMCAllEightTeV{\ensuremath{  5.97 \pm 0.17 \pm 1.01}}

\newcommand\ExpDibosMCEEEEEightTeVNoU{\ensuremath{ 0.064}}
\newcommand\ExpDibosMCEEMMEightTeVNoU{\ensuremath{ 0.156}}
\newcommand\ExpDibosMCMMEEEightTeVNoU{\ensuremath{ 0.132}}
\newcommand\ExpDibosMCMMMMEightTeVNoU{\ensuremath{ 0.301}}
\newcommand\ExpDibosMCAllEightTeVNoU{\ensuremath{ 0.653}}

\newcommand\ExpBkgSimFitEEEEEightTeV{\ensuremath{2.4 \pm 0.32 \pm 0.29  }}
\newcommand\ExpBkgSimFitEEMMEightTeV{\ensuremath{ 6.0 \pm 0.32 \pm 1.10 }}
\newcommand\ExpBkgSimFitMMEEEightTeV{\ensuremath{ 4.6 \pm 0.74 \pm 0.57  }}
\newcommand\ExpBkgSimFitMMMMEightTeV{\ensuremath{ 6.9 \pm 0.51 \pm 1.30  }}

\newcommand\ExpBkgEEEEEightTeV{\ensuremath{3.6 \pm 0.47  }}
\newcommand\ExpBkgEEMMEightTeV{\ensuremath{ 7.6 \pm 1.15 }}
\newcommand\ExpBkgMMEEEightTeV{\ensuremath{ 6.0 \pm 0.97  }}
\newcommand\ExpBkgMMMMEightTeV{\ensuremath{ 9.0 \pm 1.49  }}
\newcommand\ExpBkgAllEightTeV{\ensuremath{  26.2 \pm 2.97}}
\newcommand\ExpBkgFFIEEEEEightTeV{\ensuremath{ 3.18 \pm 0.19 \pm 0.38  }}
\newcommand\ExpBkgFFIEEMMEightTeV{\ensuremath{ 4.40 \pm 0.53 \pm 0.29  }}
\newcommand\ExpBkgFFIMMEEEightTeV{\ensuremath{ 4.22 \pm 0.26 \pm 0.48  }}
\newcommand\ExpBkgFFIMMMMEightTeV{\ensuremath{ 9.32 \pm 1.75 \pm 2.29  }}
\newcommand\ExpBkgFFIAllEightTeV{\ensuremath{ 21.13 \pm 1.88 \pm 2.45  }}
\newcommand\ExpDDEEEEFFII{\ensuremath{  2.4  \pm 0.6 \pm 0.1}}
\newcommand\ExpDDEEMMFFII{\ensuremath{  5.6  \pm 1.8 \pm 0.8}}
\newcommand\ExpDDMMEEFFII{\ensuremath{  4.4  \pm 1.0 \pm 0.3}}
\newcommand\ExpDDMMMMFFII{\ensuremath{  10.0 \pm 2.6 \pm 1.3}}
\newcommand\ExpDDAllFFII{\ensuremath{  22.4 \pm 3.4 \pm 1.6}}
\newcommand\ExpBkgFFIIEEEEEightTeV{\ensuremath{ 4.8 \pm 0.61 \pm 0.21  }}
\newcommand\ExpBkgFFIIEEMMEightTeV{\ensuremath{ 8.4 \pm 1.80 \pm 0.84  }}
\newcommand\ExpBkgFFIIMMEEEightTeV{\ensuremath{ 7.5 \pm 1.00 \pm 0.38  }}
\newcommand\ExpBkgFFIIMMMMEightTeV{\ensuremath{14.1 \pm 2.60 \pm 1.34  }}
\newcommand\ExpBkgFFIIAllEightTeV{\ensuremath{ 34.8 \pm 3.38 \pm 1.64  }}



\newcommand\UCElSmearUpEESevenTeV{\ensuremath{ 0.23\%}}
\newcommand\UCElSmearUpMMSevenTeV{\ensuremath{ 0\%}}
\newcommand\UCElSmearUpMESevenTeV{\ensuremath{ -0.08\%}}
\newcommand\UCElSmearUpEMSevenTeV{\ensuremath{ 0.21\%}}
\newcommand\UCElSmearDnEESevenTeV{\ensuremath{ -0.39\%}}
\newcommand\UCElSmearDnMMSevenTeV{\ensuremath{ 0\%}}
\newcommand\UCElSmearDnMESevenTeV{\ensuremath{ -0.29\%}}
\newcommand\UCElSmearDnEMSevenTeV{\ensuremath{ 0.28\%}}
\newcommand\UCElIdEffUpEESevenTeV{\ensuremath{ 13.82\%}}
\newcommand\UCElIdEffUpMMSevenTeV{\ensuremath{ 0\%}}
\newcommand\UCElIdEffUpMESevenTeV{\ensuremath{ 9.14\%}}
\newcommand\UCElIdEffUpEMSevenTeV{\ensuremath{ 4.07\%}}
\newcommand\UCElIdEffDnEESevenTeV{\ensuremath{ -12.56\%}}
\newcommand\UCElIdEffDnMMSevenTeV{\ensuremath{ 0\%}}
\newcommand\UCElIdEffDnMESevenTeV{\ensuremath{ -8.73\%}}
\newcommand\UCElIdEffDnEMSevenTeV{\ensuremath{ -4.00\%}}
\newcommand\UCElRecoUpEESevenTeV{\ensuremath{ 5.55\%}}
\newcommand\UCElRecoUpMMSevenTeV{\ensuremath{ 0\%}}
\newcommand\UCElRecoUpMESevenTeV{\ensuremath{ 3.51\%}}
\newcommand\UCElRecoUpEMSevenTeV{\ensuremath{ 2.00\%}}
\newcommand\UCElRecoDnEESevenTeV{\ensuremath{ -5.32\%}}
\newcommand\UCElRecoDnMMSevenTeV{\ensuremath{ 0\%}}
\newcommand\UCElRecoDnMESevenTeV{\ensuremath{ -3.45\%}}
\newcommand\UCElRecoDnEMSevenTeV{\ensuremath{ -1.98\%}}
\newcommand\UCElTrigUpEESevenTeV{\ensuremath{ 0.35\%}}
\newcommand\UCElTrigUpMMSevenTeV{\ensuremath{ 0\%}}
\newcommand\UCElTrigUpMESevenTeV{\ensuremath{ 0.06\%}}
\newcommand\UCElTrigUpEMSevenTeV{\ensuremath{ 0.29\%}}
\newcommand\UCElTrigDnEESevenTeV{\ensuremath{ -0.35\%}}
\newcommand\UCElTrigDnMMSevenTeV{\ensuremath{ 0\%}}
\newcommand\UCElTrigDnMESevenTeV{\ensuremath{ -0.06\%}}
\newcommand\UCElTrigDnEMSevenTeV{\ensuremath{ -0.29\%}}
\newcommand\UCMuMSUpEESevenTeV{\ensuremath{ 0\%}}
\newcommand\UCMuMSUpMMSevenTeV{\ensuremath{ 0.01\%}}
\newcommand\UCMuMSUpMESevenTeV{\ensuremath{ 0.07\%}}
\newcommand\UCMuMSUpEMSevenTeV{\ensuremath{ -0.02\%}}
\newcommand\UCMuMSDnEESevenTeV{\ensuremath{ 0\%}}
\newcommand\UCMuMSDnMMSevenTeV{\ensuremath{ 0.03\%}}
\newcommand\UCMuMSDnMESevenTeV{\ensuremath{ 0.06\%}}
\newcommand\UCMuMSDnEMSevenTeV{\ensuremath{ 0.08\%}}
\newcommand\UCMuIDUpEESevenTeV{\ensuremath{ 0\%}}
\newcommand\UCMuIDUpMMSevenTeV{\ensuremath{ 0.01\%}}
\newcommand\UCMuIDUpMESevenTeV{\ensuremath{ 0.12\%}}
\newcommand\UCMuIDUpEMSevenTeV{\ensuremath{ -0.03\%}}
\newcommand\UCMuIDDnEESevenTeV{\ensuremath{ 0\%}}
\newcommand\UCMuIDDnMMSevenTeV{\ensuremath{ 0.04\%}}
\newcommand\UCMuIDDnMESevenTeV{\ensuremath{ 0.06\%}}
\newcommand\UCMuIDDnEMSevenTeV{\ensuremath{ -0.03\%}}
\newcommand\UCMuScaleUpEESevenTeV{\ensuremath{ 0\%}}
\newcommand\UCMuScaleUpMMSevenTeV{\ensuremath{ 0.18\%}}
\newcommand\UCMuScaleUpMESevenTeV{\ensuremath{ 0.13\%}}
\newcommand\UCMuScaleUpEMSevenTeV{\ensuremath{ 0.14\%}}
\newcommand\UCMuScaleDnEESevenTeV{\ensuremath{ 0\%}}
\newcommand\UCMuScaleDnMMSevenTeV{\ensuremath{ -0.21\%}}
\newcommand\UCMuScaleDnMESevenTeV{\ensuremath{ 0.05\%}}
\newcommand\UCMuScaleDnEMSevenTeV{\ensuremath{ -0.21\%}}
\newcommand\UCMuIdEffUpEESevenTeV{\ensuremath{ 0\%}}
\newcommand\UCMuIdEffUpMMSevenTeV{\ensuremath{ 2.54\%}}
\newcommand\UCMuIdEffUpMESevenTeV{\ensuremath{ 0.83\%}}
\newcommand\UCMuIdEffUpEMSevenTeV{\ensuremath{ 1.76\%}}
\newcommand\UCMuIdEffDnEESevenTeV{\ensuremath{ 0\%}}
\newcommand\UCMuIdEffDnMMSevenTeV{\ensuremath{ -2.49\%}}
\newcommand\UCMuIdEffDnMESevenTeV{\ensuremath{ -0.83\%}}
\newcommand\UCMuIdEffDnEMSevenTeV{\ensuremath{ -1.74\%}}
\newcommand\UCMuTrigUpEESevenTeV{\ensuremath{ 0\%}}
\newcommand\UCMuTrigUpMMSevenTeV{\ensuremath{ 0.80\%}}
\newcommand\UCMuTrigUpMESevenTeV{\ensuremath{ 0.78\%}}
\newcommand\UCMuTrigUpEMSevenTeV{\ensuremath{ 0.07\%}}
\newcommand\UCMuTrigDnEESevenTeV{\ensuremath{ 0\%}}
\newcommand\UCMuTrigDnMMSevenTeV{\ensuremath{ -0.80\%}}
\newcommand\UCMuTrigDnMESevenTeV{\ensuremath{ -0.78\%}}
\newcommand\UCMuTrigDnEMSevenTeV{\ensuremath{ -0.07\%}}
\newcommand\UCIsoIPUpEESevenTeV{\ensuremath{ 2.24\%}}
\newcommand\UCIsoIPUpMMSevenTeV{\ensuremath{ 0.42\%}}
\newcommand\UCIsoIPUpMESevenTeV{\ensuremath{ 1.62\%}}
\newcommand\UCIsoIPUpEMSevenTeV{\ensuremath{ 0.91\%}}
\newcommand\UCIsoIPDnEESevenTeV{\ensuremath{ -2.21\%}}
\newcommand\UCIsoIPDnMMSevenTeV{\ensuremath{ -0.42\%}}
\newcommand\UCIsoIPDnMESevenTeV{\ensuremath{ -1.61\%}}
\newcommand\UCIsoIPDnEMSevenTeV{\ensuremath{ -0.91\%}}
\newcommand\UCTotalEESevenTeV{\ensuremath{ 14.46\%}}
\newcommand\UCTotalMMSevenTeV{\ensuremath{ 2.68\%}}
\newcommand\UCTotalMESevenTeV{\ensuremath{ 9.80\%}}
\newcommand\UCTotalEMSevenTeV{\ensuremath{ 4.93\%}}
\newcommand\UCElSmearUpEEEightTeV{\ensuremath{ -0.18\%}}
\newcommand\UCElSmearUpMMEightTeV{\ensuremath{ 0\%}}
\newcommand\UCElSmearUpMEEightTeV{\ensuremath{ -0.31\%}}
\newcommand\UCElSmearUpEMEightTeV{\ensuremath{ 0.07\%}}
\newcommand\UCElSmearDnEEEightTeV{\ensuremath{ 0.24\%}}
\newcommand\UCElSmearDnMMEightTeV{\ensuremath{ 0\%}}
\newcommand\UCElSmearDnMEEightTeV{\ensuremath{ -0.56\%}}
\newcommand\UCElSmearDnEMEightTeV{\ensuremath{ 0.06\%}}
\newcommand\UCElIdEffUpEEEightTeV{\ensuremath{ 6.58\%}}
\newcommand\UCElIdEffUpMMEightTeV{\ensuremath{ 0\%}}
\newcommand\UCElIdEffUpMEEightTeV{\ensuremath{ 3.76\%}}
\newcommand\UCElIdEffUpEMEightTeV{\ensuremath{ 2.66\%}}
\newcommand\UCElIdEffDnEEEightTeV{\ensuremath{ -6.27\%}}
\newcommand\UCElIdEffDnMMEightTeV{\ensuremath{ 0\%}}
\newcommand\UCElIdEffDnMEEightTeV{\ensuremath{ -3.69\%}}
\newcommand\UCElIdEffDnEMEightTeV{\ensuremath{ -2.63\%}}
\newcommand\UCElRecoUpEEEightTeV{\ensuremath{ 6.95\%}}
\newcommand\UCElRecoUpMMEightTeV{\ensuremath{ 0\%}}
\newcommand\UCElRecoUpMEEightTeV{\ensuremath{ 4.81\%}}
\newcommand\UCElRecoUpEMEightTeV{\ensuremath{ 1.58\%}}
\newcommand\UCElRecoDnEEEightTeV{\ensuremath{ -5.77\%}}
\newcommand\UCElRecoDnMMEightTeV{\ensuremath{ 0\%}}
\newcommand\UCElRecoDnMEEightTeV{\ensuremath{ -4.00\%}}
\newcommand\UCElRecoDnEMEightTeV{\ensuremath{ -1.52\%}}
\newcommand\UCElTrigUpEEEightTeV{\ensuremath{ 0.73\%}}
\newcommand\UCElTrigUpMMEightTeV{\ensuremath{ 0\%}}
\newcommand\UCElTrigUpMEEightTeV{\ensuremath{ 0.09\%}}
\newcommand\UCElTrigUpEMEightTeV{\ensuremath{ 0.66\%}}
\newcommand\UCElTrigDnEEEightTeV{\ensuremath{ -0.73\%}}
\newcommand\UCElTrigDnMMEightTeV{\ensuremath{ 0\%}}
\newcommand\UCElTrigDnMEEightTeV{\ensuremath{ -0.09\%}}
\newcommand\UCElTrigDnEMEightTeV{\ensuremath{ -0.66\%}}
\newcommand\UCMuMSUpEEEightTeV{\ensuremath{ 0\%}}
\newcommand\UCMuMSUpMMEightTeV{\ensuremath{ -0.05\%}}
\newcommand\UCMuMSUpMEEightTeV{\ensuremath{ -0.07\%}}
\newcommand\UCMuMSUpEMEightTeV{\ensuremath{ -0.01\%}}
\newcommand\UCMuMSDnEEEightTeV{\ensuremath{ 0\%}}
\newcommand\UCMuMSDnMMEightTeV{\ensuremath{ -0.03\%}}
\newcommand\UCMuMSDnMEEightTeV{\ensuremath{ 0.00\%}}
\newcommand\UCMuMSDnEMEightTeV{\ensuremath{ 0.01\%}}
\newcommand\UCMuIDUpEEEightTeV{\ensuremath{ 0\%}}
\newcommand\UCMuIDUpMMEightTeV{\ensuremath{ -0.02\%}}
\newcommand\UCMuIDUpMEEightTeV{\ensuremath{ 0.02\%}}
\newcommand\UCMuIDUpEMEightTeV{\ensuremath{ 0.01\%}}
\newcommand\UCMuIDDnEEEightTeV{\ensuremath{ 0\%}}
\newcommand\UCMuIDDnMMEightTeV{\ensuremath{ -0.01\%}}
\newcommand\UCMuIDDnMEEightTeV{\ensuremath{ 0.02\%}}
\newcommand\UCMuIDDnEMEightTeV{\ensuremath{ -0.01\%}}
\newcommand\UCMuScaleUpEEEightTeV{\ensuremath{ 0\%}}
\newcommand\UCMuScaleUpMMEightTeV{\ensuremath{ 0.28\%}}
\newcommand\UCMuScaleUpMEEightTeV{\ensuremath{ -0.02\%}}
\newcommand\UCMuScaleUpEMEightTeV{\ensuremath{ 0.28\%}}
\newcommand\UCMuScaleDnEEEightTeV{\ensuremath{ 0\%}}
\newcommand\UCMuScaleDnMMEightTeV{\ensuremath{ -0.36\%}}
\newcommand\UCMuScaleDnMEEightTeV{\ensuremath{ -0.02\%}}
\newcommand\UCMuScaleDnEMEightTeV{\ensuremath{ -0.29\%}}
\newcommand\UCMuIdEffUpEEEightTeV{\ensuremath{ 0\%}}
\newcommand\UCMuIdEffUpMMEightTeV{\ensuremath{ 2.47\%}}
\newcommand\UCMuIdEffUpMEEightTeV{\ensuremath{ 0.80\%}}
\newcommand\UCMuIdEffUpEMEightTeV{\ensuremath{ 1.75\%}}
\newcommand\UCMuIdEffDnEEEightTeV{\ensuremath{ 0\%}}
\newcommand\UCMuIdEffDnMMEightTeV{\ensuremath{ -2.43\%}}
\newcommand\UCMuIdEffDnMEEightTeV{\ensuremath{ -0.80\%}}
\newcommand\UCMuIdEffDnEMEightTeV{\ensuremath{ -1.74\%}}
\newcommand\UCMuTrigUpEEEightTeV{\ensuremath{ 0\%}}
\newcommand\UCMuTrigUpMMEightTeV{\ensuremath{ 1.01\%}}
\newcommand\UCMuTrigUpMEEightTeV{\ensuremath{ 0.94\%}}
\newcommand\UCMuTrigUpEMEightTeV{\ensuremath{ 0.06\%}}
\newcommand\UCMuTrigDnEEEightTeV{\ensuremath{ 0\%}}
\newcommand\UCMuTrigDnMMEightTeV{\ensuremath{ -1.01\%}}
\newcommand\UCMuTrigDnMEEightTeV{\ensuremath{ -0.94\%}}
\newcommand\UCMuTrigDnEMEightTeV{\ensuremath{ -0.06\%}}
\newcommand\UCIsoIPUpEEEightTeV{\ensuremath{ 2.24\%}}
\newcommand\UCIsoIPUpMMEightTeV{\ensuremath{ 0.42\%}}
\newcommand\UCIsoIPUpMEEightTeV{\ensuremath{ 1.63\%}}
\newcommand\UCIsoIPUpEMEightTeV{\ensuremath{ 0.90\%}}
\newcommand\UCIsoIPDnEEEightTeV{\ensuremath{ -2.20\%}}
\newcommand\UCIsoIPDnMMEightTeV{\ensuremath{ -0.42\%}}
\newcommand\UCIsoIPDnMEEightTeV{\ensuremath{ -1.62\%}}
\newcommand\UCIsoIPDnEMEightTeV{\ensuremath{ -0.89\%}}
\newcommand\UCTotalEEEightTeV{\ensuremath{ 4.94\%}}
\newcommand\UCTotalEMEightTeV{\ensuremath{ 2.36\%}}
\newcommand\UCTotalMEEightTeV{\ensuremath{ 3.08\%}}
\newcommand\UCTotalMMEightTeV{\ensuremath{ 1.90\%}}

\newcommand\UCTotalEESevenTeVSummary{\ensuremath{ 14.5\%}}
\newcommand\UCTotalMMSevenTeVSummary{\ensuremath{ 2.7\%}}
\newcommand\UCTotalMESevenTeVSummary{\ensuremath{ 9.8\%}}
\newcommand\UCTotalEMSevenTeVSummary{\ensuremath{ 4.9\%}}
\newcommand\UCTotalEEEightTeVSummary{\ensuremath{ 9.4\%}}
\newcommand\UCTotalMMEightTeVSummary{\ensuremath{ 2.7\%}}
\newcommand\UCTotalMEEightTeVSummary{\ensuremath{ 6.2\%}}
\newcommand\UCTotalEMEightTeVSummary{\ensuremath{ 3.7\%}}

\newcommand\CzfourlEEEESevenTeV{\ensuremath{ 21.5\%}}
\newcommand\CzfourlEEMMSevenTeV{\ensuremath{ 49.0\%}}
\newcommand\CzfourlMMEESevenTeV{\ensuremath{ 36.3\%}}
\newcommand\CzfourlMMMMSevenTeV{\ensuremath{ 59.2\%}}
\newcommand\AltCzfourlEEEEEightTeV{\ensuremath{ 53.68\%}}
\newcommand\AltCzfourlEEMMEightTeV{\ensuremath{ 67.02\%}}
\newcommand\AltCzfourlMMEEEightTeV{\ensuremath{ 69.01\%}}
\newcommand\AltCzfourlMMMMEightTeV{\ensuremath{ 82.45\%}}
\newcommand\CzfourlEEEEEightTeV{\ensuremath{ 53.28\%}}
\newcommand\CzfourlEEMMEightTeV{\ensuremath{ 66.90\%}}
\newcommand\CzfourlMMEEEightTeV{\ensuremath{ 68.58\%}}
\newcommand\CzfourlMMMMEightTeV{\ensuremath{ 82.18\%}}
\newcommand\DeltaBOverSigEESevenTeV{\ensuremath{ 5.68\%}}
\newcommand\DeltaBOverSigEMSevenTeV{\ensuremath{ 1.32\%}}
\newcommand\DeltaBOverSigMESevenTeV{\ensuremath{ 0.61\%}}
\newcommand\DeltaBOverSigMMSevenTeV{\ensuremath{ 0.51\%}}
\newcommand\FidSigmaErrorEESevenTeV{\ensuremath{ 15.54\%}}
\newcommand\FidSigmaErrorEMSevenTeV{\ensuremath{ 5.10\%}}
\newcommand\FidSigmaErrorMESevenTeV{\ensuremath{ 9.82\%}}
\newcommand\FidSigmaErrorMMSevenTeV{\ensuremath{ 2.73\%}}
\newcommand\DeltaBOverSigEEEightTeV{\ensuremath{ 0.10\%}}
\newcommand\DeltaBOverSigEMEightTeV{\ensuremath{ 0.12\%}}
\newcommand\DeltaBOverSigMEEightTeV{\ensuremath{ 0.19\%}}
\newcommand\DeltaBOverSigMMEightTeV{\ensuremath{ 0.08\%}}
\newcommand\FidSigmaErrorEEEightTeV{\ensuremath{ 9.36\%}}
\newcommand\FidSigmaErrorEMEightTeV{\ensuremath{ 3.71\%}}
\newcommand\FidSigmaErrorMEEightTeV{\ensuremath{ 6.15\%}}
\newcommand\FidSigmaErrorMMEightTeV{\ensuremath{ 2.70\%}}


\newcommand\FiducialXsecTheoryEEEESevenTeV{\ensuremath{ 1.70 \pm 0.04\text{ fb}}}
\newcommand\FiducialXsecTheoryEEMMSevenTeV{\ensuremath{ 3.50 \pm 0.01\text{ fb}}}
\newcommand\FiducialXsecTheoryMMEESevenTeV{\ensuremath{ 1.94 \pm 0.01\text{ fb}}}
\newcommand\FiducialXsecTheoryMMMMSevenTeV{\ensuremath{ 4.18 \pm 0.01\text{ fb}}}
\newcommand\FiducialXsecTheoryAllSevenTeV{\ensuremath{ 69.6 \pm 1.6\text{ fb}}}
\newcommand\FiducialXsecTheoryEESMMSevenTeV{\ensuremath{ 35.6 \pm 0.8\text{ fb}}}
\newcommand\FiducialXsecTheoryEEMMSMMEESevenTeV{\ensuremath{ 33.9 \pm 0.8\text{ fb}}}
\newcommand\FiducialXsecTheoryEEEEEightTeV{\ensuremath{ 1.95 \pm 0.05\text{ fb}}}
\newcommand\FiducialXsecTheoryEEMMEightTeV{\ensuremath{ 3.81 \pm 0.09\text{ fb}}}
\newcommand\FiducialXsecTheoryMMEEEightTeV{\ensuremath{ 2.04 \pm 0.05\text{ fb}}}
\newcommand\FiducialXsecTheoryMMMMEightTeV{\ensuremath{ 4.74 \pm 0.12\text{ fb}}}
\newcommand\FiducialXsecTheoryAllEightTeV{\ensuremath{ 79.2 \pm 1.9\text{ fb}}}
\newcommand\FiducialXsecTheoryEESMMEightTeV{\ensuremath{ 40.6 \pm 1.0\text{ fb}}}
\newcommand\FiducialXsecTheoryEEMMSMMEEEightTeV{\ensuremath{ 38.5 \pm 0.9\text{ fb}}}


\newcommand\FiducialXsecObsEEEESevenTeV{\ensuremath{ 0.910^{+1.39}_{-0.72}\text{ (stat)} \pm 0.14\text{ (syst)} \pm 0.02\text{ (lumi)}\text{ fb}}}
\newcommand\FiducialXsecObsEEMMSevenTeV{\ensuremath{ 3.091^{+1.35}_{-1.05}\text{ (stat)} \pm 0.16\text{ (syst)} \pm 0.05\text{ (lumi)}\text{ fb}}}
\newcommand\FiducialXsecObsMMEESevenTeV{\ensuremath{ 3.015^{+1.57}_{-1.17}\text{ (stat)} \pm 0.30\text{ (syst)} \pm 0.06\text{ (lumi)}\text{ fb}}}
\newcommand\FiducialXsecObsMMMMSevenTeV{\ensuremath{ 2.970^{+1.18}_{-0.94}\text{ (stat)} \pm 0.07\text{ (syst)} \pm 0.05\text{ (lumi)}\text{ fb}}}
\newcommand\FiducialXsecObsEEEEEightTeV{\ensuremath{ 7.41 \pm 0.85\text{ (stat)} \pm 0.37\text{ (syst)} \pm 0.21\text{ (lumi)}\text{ fb}}}
\newcommand\FiducialXsecObsEEMMEightTeV{\ensuremath{ 9.43 \pm 0.86\text{ (stat)} \pm 0.23\text{ (syst)} \pm 0.26\text{ (lumi)}\text{ fb}}}
\newcommand\FiducialXsecObsMMEEEightTeV{\ensuremath{ 6.56 \pm 0.72\text{ (stat)} \pm 0.21\text{ (syst)} \pm 0.18\text{ (lumi)}\text{ fb}}}
\newcommand\FiducialXsecObsMMMMEightTeV{\ensuremath{ 8.70 \pm 0.75\text{ (stat)} \pm 0.17\text{ (syst)} \pm 0.24\text{ (lumi)}\text{ fb}}}
\newcommand\FiducialLLXsecObsEEEESevenTeV{\ensuremath{ 0.9^{+1.4}_{-0.7}\text{ (stat)}^{+0.3}_{-0.04}\text{ (syst)}\text{ fb}}}
\newcommand\FiducialLLXsecObsEEMMSevenTeV{\ensuremath{ 3.1^{+1.4}_{-1.0}\text{ (stat)}^{+0.2}_{-0.04}\text{ (syst)}\text{ fb}}}
\newcommand\FiducialLLXsecObsMMEESevenTeV{\ensuremath{ 3.0^{+1.6}_{-1.2}\text{ (stat)}^{+0.4}_{-0.2}\text{ (syst)}\text{ fb}}}
\newcommand\FiducialLLXsecObsMMMMSevenTeV{\ensuremath{ 3.0^{+1.2}_{-0.9}\text{ (stat)}^{+0.1}_{-0.08}\text{ (syst)}\text{ fb}}}
\newcommand\FiducialLLXsecObsEEEEEightTeV{\ensuremath{ 2.2^{+0.6}_{-0.5}\text{ (stat)}^{+0.2}_{-0.1}\text{ (syst)}\text{ fb}}}
\newcommand\FiducialLLXsecObsEEMMEightTeV{\ensuremath{ 4.2^{+0.6}_{-0.6}\text{ (stat)}^{+0.2}_{-0.2}\text{ (syst)}\text{ fb}}}
\newcommand\FiducialLLXsecObsMMEEEightTeV{\ensuremath{ 1.7^{+0.4}_{-0.4}\text{ (stat)}^{+0.2}_{-0.1}\text{ (syst)}\text{ fb}}}
\newcommand\FiducialLLXsecObsMMMMEightTeV{\ensuremath{ 4.9^{+0.6}_{-0.6}\text{ (stat)}^{+0.1}_{-0.1}\text{ (syst)}\text{ fb}}}

\newcommand\FiducialXsecObsEEEESevenTeVPlain{\ensuremath{ 0.910^{+1.39}_{-0.72} \pm 0.14 \pm 0.02}}
\newcommand\FiducialXsecObsEEMMSevenTeVPlain{\ensuremath{ 3.091^{+1.35}_{-1.05} \pm 0.16 \pm 0.05}}
\newcommand\FiducialXsecObsMMEESevenTeVPlain{\ensuremath{ 3.015^{+1.57}_{-1.17} \pm 0.30 \pm 0.06}}
\newcommand\FiducialXsecObsMMMMSevenTeVPlain{\ensuremath{ 2.970^{+1.18}_{-0.94} \pm 0.07 \pm 0.05}}
\newcommand\FiducialXsecObsEEEEEightTeVPlain{\ensuremath{ 2.16^{+0.59}_{-0.50} \pm 0.20 \pm 0.06}}
\newcommand\FiducialXsecObsEEMMEightTeVPlain{\ensuremath{ 4.23^{+0.65}_{-0.59} \pm 0.16 \pm 0.12}}
\newcommand\FiducialXsecObsMMEEEightTeVPlain{\ensuremath{ 1.68^{+0.46}_{-0.39} \pm 0.10 \pm 0.04}}
\newcommand\FiducialXsecObsMMMMEightTeVPlain{\ensuremath{ 4.89^{+0.66}_{-0.56} \pm 0.13 \pm 0.14}}
\newcommand\FiducialLikelihoodXsecObsEEEESevenTeVPlain{\ensuremath{ 0.91^{+1.42}_{0.70} \pm 0.18 \pm 0.02}}
\newcommand\FiducialLikelihoodXsecObsEEMMSevenTeVPlain{\ensuremath{ 3.09^{+1.36}_{1.05} \pm 0.17 \pm 0.06}}
\newcommand\FiducialLikelihoodXsecObsMMEESevenTeVPlain{\ensuremath{ 3.01^{+1.61}_{1.14} \pm 0.31 \pm 0.06}}
\newcommand\FiducialLikelihoodXsecObsMMMMSevenTeVPlain{\ensuremath{ 2.97^{+1.19}_{0.94} \pm 0.08 \pm 0.06}}
\newcommand\FiducialLikelihoodXsecObsEEEEEightTeVPlain{\ensuremath{ 2.16^{+0.60}_{0.49} \pm 0.20 \pm 0.06}}
\newcommand\FiducialLikelihoodXsecObsEEMMEightTeVPlain{\ensuremath{ 4.22^{+0.66}_{0.57} \pm 0.16 \pm 0.12}}
\newcommand\FiducialLikelihoodXsecObsMMEEEightTeVPlain{\ensuremath{ 1.68^{+0.47}_{0.39} \pm 0.11 \pm 0.05}}
\newcommand\FiducialLikelihoodXsecObsMMMMEightTeVPlain{\ensuremath{ 4.89^{+0.61}_{0.55} \pm 0.13 \pm 0.14}}
\newcommand\PhaseSpaceLikelihoodXsecObsEEEESevenTeVPlain{\ensuremath{ 12.18^{+19.04}_{9.37} \pm 2.48 \pm 0.28}}
\newcommand\PhaseSpaceLikelihoodXsecObsEEMMSevenTeVPlain{\ensuremath{ 19.53^{+8.61}_{6.59} \pm 1.08 \pm 0.36}}
\newcommand\PhaseSpaceLikelihoodXsecObsMMEESevenTeVPlain{\ensuremath{ 34.26^{+18.27}_{13.02} \pm 3.61 \pm 0.65}}
\newcommand\PhaseSpaceLikelihoodXsecObsMMMMSevenTeVPlain{\ensuremath{ 16.26^{+6.52}_{5.13} \pm 0.50 \pm 0.30}}
\newcommand\PhaseSpaceLikelihoodXsecObsMixSevenTeVPlain{\ensuremath{ 47.45^{+15.59}_{12.58} \pm 2.80 \pm 0.87}}
\newcommand\PhaseSpaceLikelihoodXsecObsSameSevenTeVPlain{\ensuremath{ 31.55^{+12.00}_{9.52} \pm 1.08 \pm 0.58}}
\newcommand\PhaseSpaceLikelihoodXsecObsSevenTeVPlain{\ensuremath{ 79.05^{+19.18}_{16.20} \pm 3.81 \pm 1.44}}
\newcommand\PhaseSpaceLikelihoodXsecObsEEEEEightTeVPlain{\ensuremath{ 29.64^{+8.27}_{6.71} \pm 2.86 \pm 0.85}}
\newcommand\PhaseSpaceLikelihoodXsecObsEEMMEightTeVPlain{\ensuremath{ 28.55^{+4.41}_{3.89} \pm 1.16 \pm 0.81}}
\newcommand\PhaseSpaceLikelihoodXsecObsMMEEEightTeVPlain{\ensuremath{ 21.27^{+5.89}_{4.89} \pm 1.36 \pm 0.61}}
\newcommand\PhaseSpaceLikelihoodXsecObsMMMMEightTeVPlain{\ensuremath{ 27.48^{+3.45}_{3.11} \pm 0.83 \pm 0.77}}
\newcommand\PhaseSpaceLikelihoodXsecObsMixEightTeVPlain{\ensuremath{ 52.69^{+7.01}_{6.26} \pm 2.46 \pm 1.49}}
\newcommand\PhaseSpaceLikelihoodXsecObsSameEightTeVPlain{\ensuremath{ 55.69^{+6.30}_{5.71} \pm 1.83 \pm 1.57}}
\newcommand\PhaseSpaceLikelihoodXsecObsEightTeVPlain{\ensuremath{ 108.26^{+9.39}_{8.50} \pm 3.99 \pm 3.05}}
\newcommand\AltPhaseSpaceXsecObsEEEESevenTeVPlain{\ensuremath{ 16.69^{+25.61}_{-13.17} \pm 3.67 \pm 0.30}}
\newcommand\AltPhaseSpaceXsecObsMMMMSevenTeVPlain{\ensuremath{ 22.21^{+8.86}_{-7.00} \pm 0.66 \pm 0.40}}
\newcommand\AltPhaseSpaceXsecObsEEMMSevenTeVPlain{\ensuremath{ 26.42^{+11.53}_{-8.96} \pm 1.39 \pm 0.47}}
\newcommand\AltPhaseSpaceXsecObsMMEESevenTeVPlain{\ensuremath{ 46.38^{+24.19}_{-17.95} \pm 4.59 \pm 0.83}}
\newcommand\AltPhaseSpaceXsecObsEEEEEightTeVPlain{\ensuremath{ 40.51^{+10.64}_{-9.01} \pm 3.91 \pm 1.08}}
\newcommand\AltPhaseSpaceXsecObsMMMMEightTeVPlain{\ensuremath{ 37.52^{+4.77}_{-4.40} \pm 1.12 \pm 1.06}}
\newcommand\AltPhaseSpaceXsecObsEEMMEightTeVPlain{\ensuremath{ 38.63^{+5.81}_{-5.27} \pm 1.55 \pm 1.05}}
\newcommand\AltPhaseSpaceXsecObsMMEEEightTeVPlain{\ensuremath{ 28.70^{+7.50}_{-6.31} \pm 1.82 \pm 0.74}}
\newcommand\PhaseSpaceXsecObsEEEESevenTeVPlain{\ensuremath{ 12.17^{+18.67}_{-9.60} \pm 2.68 \pm 0.22}}
\newcommand\PhaseSpaceXsecObsMMMMSevenTeVPlain{\ensuremath{ 16.26^{+6.49}_{-5.12} \pm 0.48 \pm 0.29}}
\newcommand\PhaseSpaceXsecObsEEMMSevenTeVPlain{\ensuremath{ 19.52^{+8.52}_{-6.62} \pm 1.03 \pm 0.35}}
\newcommand\PhaseSpaceXsecObsMMEESevenTeVPlain{\ensuremath{ 34.29^{+17.88}_{-13.27} \pm 3.39 \pm 0.61}}
\newcommand\PhaseSpaceXsecObsEEEEEightTeVPlain{\ensuremath{ 18.33^{+7.79}_{-6.59} \pm 2.86 \pm 0.79}}
\newcommand\PhaseSpaceXsecObsMMMMEightTeVPlain{\ensuremath{ 18.25^{+3.49}_{-3.22} \pm 0.82 \pm 0.78}}
\newcommand\PhaseSpaceXsecObsEEMMEightTeVPlain{\ensuremath{ 23.62^{+4.30}_{-3.90} \pm 1.15 \pm 0.78}}
\newcommand\PhaseSpaceXsecObsMMEEEightTeVPlain{\ensuremath{ 16.95^{+5.56}_{-4.68} \pm 1.35 \pm 0.55}}
\newcommand\AltPhaseSpaceXsecObsMixSevenTeVPlain{\ensuremath{ 60.0 \pm 18.7 \pm 4.5 \pm 1.2}}
\newcommand\AltPhaseSpaceXsecObsSameSevenTeVPlain{\ensuremath{ 42.9 \pm 14.9 \pm 1.3 \pm 0.8}}
\newcommand\AltPhaseSpaceXsecObsSevenTeVPlain{\ensuremath{ 102.9 \pm 23.0 \pm 4.4 \pm 1.9}}
\newcommand\AltPhaseSpaceXsecObsMixEightTeVPlain{\ensuremath{ 69.7 \pm 8.8 \pm 3.2 \pm 2.0}}
\newcommand\AltPhaseSpaceXsecObsSameEightTeVPlain{\ensuremath{ 76.0 \pm 8.2 \pm 2.5 \pm 2.1}}
\newcommand\AltPhaseSpaceXsecObsEightTeVPlain{\ensuremath{ 145.3 \pm 12.0 \pm 5.4 \pm 4.1}}
\newcommand\PhaseSpaceXsecObsMixSevenTeVPlain{\ensuremath{ 44.3 \pm 13.8 \pm 3.3 \pm 0.9}}
\newcommand\PhaseSpaceXsecObsSameSevenTeVPlain{\ensuremath{ 31.4 \pm 10.9 \pm 1.0 \pm 0.6}}
\newcommand\PhaseSpaceXsecObsSevenTeVPlain{\ensuremath{ 75.8 \pm 17.6 \pm 4.0 \pm 1.4}}
\newcommand\PhaseSpaceXsecObsMixEightTeVPlain{\ensuremath{ 51.7 \pm 6.5 \pm 2.4 \pm 1.5}}
\newcommand\PhaseSpaceXsecObsSameEightTeVPlain{\ensuremath{ 55.6 \pm 6.0 \pm 1.8 \pm 1.6}}
\newcommand\PhaseSpaceXsecObsEightTeVPlain{\ensuremath{ 107.3 \pm 8.8 \pm 4.0 \pm 3.0}}

\newcommand\ChiSqSameSevenTeV{\ensuremath{ 0.06}}
\newcommand\ChiSqMixSevenTeV{\ensuremath{ 1.17}}
\newcommand\ChiSqSevenTeV{\ensuremath{ 1.23}}
\newcommand\ChiSqSameEightTeV{\ensuremath{ 0.07}}
\newcommand\ChiSqMixEightTeV{\ensuremath{ 0.69}}
\newcommand\ChiSqEightTeV{\ensuremath{ 0.77}}
\newcommand\PValueSameSevenTeV{\ensuremath{ 0.80}}
\newcommand\PValueMixSevenTeV{\ensuremath{ 0.28}}
\newcommand\PValueSevenTeV{\ensuremath{ 0.41}}
\newcommand\PValueSameEightTeV{\ensuremath{ 0.79}}
\newcommand\PValueMixEightTeV{\ensuremath{ 0.41}}
\newcommand\PValueEightTeV{\ensuremath{ 0.54}}

\newcommand\UAPDFUpEESevenTeV{\ensuremath{ 0.06\%}}
\newcommand\UAEigvecUpEESevenTeV{\ensuremath{ 1.64\%}}
\newcommand\UAScaleUpEESevenTeV{\ensuremath{ 0.30\%}}
\newcommand\UAPDFUpEMSevenTeV{\ensuremath{ 0.05\%}}
\newcommand\UAEigvecUpEMSevenTeV{\ensuremath{ 1.58\%}}
\newcommand\UAScaleUpEMSevenTeV{\ensuremath{ 0.06\%}}
\newcommand\UAPDFUpMESevenTeV{\ensuremath{ 0.05\%}}
\newcommand\UAEigvecUpMESevenTeV{\ensuremath{ 1.58\%}}
\newcommand\UAScaleUpMESevenTeV{\ensuremath{ 0.06\%}}
\newcommand\UAPDFUpMMSevenTeV{\ensuremath{ 0.10\%}}
\newcommand\UAEigvecUpMMSevenTeV{\ensuremath{ 1.33\%}}
\newcommand\UAScaleUpMMSevenTeV{\ensuremath{ 0.37\%}}
\newcommand\UATotalEESevenTeV{\ensuremath{ 1.66\%}}
\newcommand\UATotalEMSevenTeV{\ensuremath{ 1.58\%}}
\newcommand\UATotalMESevenTeV{\ensuremath{ 1.58\%}}
\newcommand\UATotalMMSevenTeV{\ensuremath{ 1.34\%}}
\newcommand\UAPDFUpEEEightTeV{\ensuremath{ 0.16\%}}
\newcommand\UAEigvecUpEEEightTeV{\ensuremath{ 1.68\%}}
\newcommand\UAScaleUpEEEightTeV{\ensuremath{ 0.10\%}}
\newcommand\UAPDFUpEMEightTeV{\ensuremath{ 0.14\%}}
\newcommand\UAEigvecUpEMEightTeV{\ensuremath{ 1.58\%}}
\newcommand\UAScaleUpEMEightTeV{\ensuremath{ 0.06\%}}
\newcommand\UAPDFUpMEEightTeV{\ensuremath{ 0.14\%}}
\newcommand\UAEigvecUpMEEightTeV{\ensuremath{ 1.58\%}}
\newcommand\UAScaleUpMEEightTeV{\ensuremath{ 0.06\%}}
\newcommand\UAPDFUpMMEightTeV{\ensuremath{ 0.01\%}}
\newcommand\UAEigvecUpMMEightTeV{\ensuremath{ 1.48\%}}
\newcommand\UAScaleUpMMEightTeV{\ensuremath{ 0.42\%}}
\newcommand\UATotalEEEightTeV{\ensuremath{ 5.02\%}}
\newcommand\UATotalEMEightTeV{\ensuremath{ 4.94\%}}
\newcommand\UATotalMEEightTeV{\ensuremath{ 5.46\%}}
\newcommand\UATotalMMEightTeV{\ensuremath{ 3.93\%}}
\newcommand\UACTotalEEEightTeV{\ensuremath{ 7.64\%}}
\newcommand\UACTotalEMEightTeV{\ensuremath{ 5.65\%}}
\newcommand\UACTotalMEEightTeV{\ensuremath{ 6.87\%}}
\newcommand\UACTotalMMEightTeV{\ensuremath{ 4.68\%}}
\newcommand\AltAzfourlEEEESevenTeV{\ensuremath{ 5.45\%}}
\newcommand\AltAzfourlMMMMSevenTeV{\ensuremath{ 13.37\%}}
\newcommand\AltAzfourlEEMMSevenTeV{\ensuremath{ 11.70\%}}
\newcommand\AltAzfourlMMEESevenTeV{\ensuremath{ 6.50\%}}
\newcommand\AltAzfourlEEEEEightTeV{\ensuremath{ 43.57\%}}
\newcommand\AltAzfourlEEMMEightTeV{\ensuremath{ 45.09\%}}
\newcommand\AltAzfourlMMEEEightTeV{\ensuremath{ 43.46\%}}
\newcommand\AltAzfourlMMMMEightTeV{\ensuremath{ 52.18\%}}
\newcommand\AzfourlEEEESevenTeV{\ensuremath{ 7.47\%}}
\newcommand\AzfourlMMMMSevenTeV{\ensuremath{ 18.26\%}}
\newcommand\AzfourlEEMMSevenTeV{\ensuremath{ 15.83\%}}
\newcommand\AzfourlMMEESevenTeV{\ensuremath{ 8.79\%}}
\newcommand\AzfourlEEEEEightTeV{\ensuremath{ 41.55\%}}
\newcommand\AzfourlEEMMEightTeV{\ensuremath{ 43.06\%}}
\newcommand\AzfourlMMEEEightTeV{\ensuremath{ 41.32\%}}
\newcommand\AzfourlMMMMEightTeV{\ensuremath{ 50.27\%}}
\newcommand\AltACzfourlEEEEEightTeV{\ensuremath{ 23.39\%}}
\newcommand\AltACzfourlEEMMEightTeV{\ensuremath{ 30.22\%}}
\newcommand\AltACzfourlMMEEEightTeV{\ensuremath{ 30.00\%}}
\newcommand\AltACzfourlMMMMEightTeV{\ensuremath{ 43.02\%}}
\newcommand\ACzfourlEEEEEightTeV{\ensuremath{ 22.14\%}}
\newcommand\ACzfourlEEMMEightTeV{\ensuremath{ 28.81\%}}
\newcommand\ACzfourlMMEEEightTeV{\ensuremath{ 28.34\%}}
\newcommand\ACzfourlMMMMEightTeV{\ensuremath{ 41.31\%}}

\newcommand\PhaseSpaceXsecObsEEEESevenTeV{\ensuremath{ 12.17^{+18.67}_{-9.60}\text{ (stat)} \pm 2.68\text{ (syst)} \pm 0.22\text{ (lumi)}\text{ fb}}}
\newcommand\PhaseSpaceXsecObsMMMMSevenTeV{\ensuremath{ 16.26^{+6.49}_{-5.12}\text{ (stat)} \pm 0.48\text{ (syst)} \pm 0.29\text{ (lumi)}\text{ fb}}}
\newcommand\PhaseSpaceXsecObsEEMMSevenTeV{\ensuremath{ 19.52^{+8.52}_{-6.62}\text{ (stat)} \pm 1.03\text{ (syst)} \pm 0.35\text{ (lumi)}\text{ fb}}}
\newcommand\PhaseSpaceXsecObsMMEESevenTeV{\ensuremath{ 34.29^{+17.88}_{-13.27}\text{ (stat)} \pm 3.39\text{ (syst)} \pm 0.61\text{ (lumi)}\text{ fb}}}
\newcommand\PhaseSpaceXsecObsEEEEEightTeV{\ensuremath{ 17.82 \pm 2.06\text{ (stat)} \pm 1.34\text{ (syst)} \pm 0.50\text{ (lumi)}\text{ fb}}}
\newcommand\PhaseSpaceXsecObsEEMMEightTeV{\ensuremath{ 21.91 \pm 2.00\text{ (stat)} \pm 1.20\text{ (syst)} \pm 0.61\text{ (lumi)}\text{ fb}}}
\newcommand\PhaseSpaceXsecObsMMEEEightTeV{\ensuremath{ 15.88 \pm 1.74\text{ (stat)} \pm 1.05\text{ (syst)} \pm 0.45\text{ (lumi)}\text{ fb}}}
\newcommand\PhaseSpaceXsecObsMMMMEightTeV{\ensuremath{ 17.30 \pm 1.49\text{ (stat)} \pm 0.79\text{ (syst)} \pm 0.48\text{ (lumi)}\text{ fb}}}
\newcommand\PhaseSpaceXsecObsMixSevenTeV{\ensuremath{ 44.3 \pm 13.8\text{ (stat)} \pm 3.3\text{ (syst)} \pm 0.9\text{ (lumi)}\text{ fb}}}
\newcommand\PhaseSpaceXsecObsSameSevenTeV{\ensuremath{ 31.4 \pm 10.9\text{ (stat)} \pm 1.0\text{ (syst)} \pm 0.6\text{ (lumi)}\text{ fb}}}
\newcommand\PhaseSpaceXsecObsSevenTeV{\ensuremath{ 75.8 \pm 17.6\text{ (stat)} \pm 4.0\text{ (syst)} \pm 1.4\text{ (lumi)}\text{ fb}}}
\newcommand\PhaseSpaceXsecObsSameEightTeV{\ensuremath{ 34.90 \pm 2.42\text{ (stat)} \pm 1.84\text{ (syst)} \pm 0.98\text{ (lumi)}\text{ fb}}}
\newcommand\PhaseSpaceXsecObsMixEightTeV{\ensuremath{  36.51 \pm 2.62\text{ (stat)} \pm 2.30\text{ (syst)} \pm 1.02\text{ (lumi)}\text{ fb}}}
\newcommand\PhaseSpaceXsecObsEightTeV{\ensuremath{     71.40 \pm 3.56\text{ (stat)} \pm 4.08\text{ (syst)} \pm 1.99\text{ (lumi)}\text{ fb}}}
\newcommand\FiducialXsecObsSameEightTeV{\ensuremath{ 16.11 \pm 1.13\text{ (stat)} \pm 0.36\text{ (syst)} \pm 0.46\text{ (lumi)}\text{ fb}}}
\newcommand\FiducialXsecObsMixEightTeV{\ensuremath{  15.99 \pm 1.10\text{ (stat)} \pm 0.39\text{ (syst)} \pm 0.43\text{ (lumi)}\text{ fb}}}
\newcommand\FiducialXsecObsEightTeV{\ensuremath{     32.10 \pm 1.58\text{ (stat)} \pm 0.74\text{ (syst)} \pm 0.89\text{ (lumi)}\text{ fb}}}

\newcommand\AltPhaseSpaceXsecTheoryEEEESevenTeV{\ensuremath{ 31.27 \pm 0.70\text{ fb}}}
\newcommand\AltPhaseSpaceXsecTheoryEEMMSevenTeV{\ensuremath{ 29.89 \pm 0.67\text{ fb}}}
\newcommand\AltPhaseSpaceXsecTheoryMMEESevenTeV{\ensuremath{ 29.89 \pm 0.67\text{ fb}}}
\newcommand\AltPhaseSpaceXsecTheoryMMMMSevenTeV{\ensuremath{ 31.27 \pm 0.70\text{ fb}}}
\newcommand\AltPhaseSpaceXsecTheorySameSevenTeV{\ensuremath{ 62.53 \pm 1.50\text{ fb}}}
\newcommand\AltPhaseSpaceXsecTheoryMixSevenTeV{\ensuremath{ 59.77 \pm 1.40\text{ fb}}}
\newcommand\AltPhaseSpaceXsecTheorySevenTeV{\ensuremath{ 122.30 \pm 2.80\text{ fb}}}
\newcommand\AltPhaseSpaceXsecTheoryEEEEEightTeV{\ensuremath{ 36.45 \pm 0.90\text{ fb}}}
\newcommand\AltPhaseSpaceXsecTheoryEEMMEightTeV{\ensuremath{ 34.79 \pm 0.86\text{ fb}}}
\newcommand\AltPhaseSpaceXsecTheoryMMEEEightTeV{\ensuremath{ 34.79 \pm 0.86\text{ fb}}}
\newcommand\AltPhaseSpaceXsecTheoryMMMMEightTeV{\ensuremath{ 36.45 \pm 0.90\text{ fb}}}
\newcommand\AltPhaseSpaceXsecTheorySameEightTeV{\ensuremath{ 72.89 \pm 1.70\text{ fb}}}
\newcommand\AltPhaseSpaceXsecTheoryMixEightTeV{\ensuremath{ 69.58 \pm 1.70\text{ fb}}}
\newcommand\AltPhaseSpaceXsecTheoryEightTeV{\ensuremath{ 142.50 \pm 3.40\text{ fb}}}
\newcommand\PhaseSpaceXsecTheoryEEEESevenTeV{\ensuremath{ 22.89 \pm 0.51\text{ fb}}}
\newcommand\PhaseSpaceXsecTheoryEEMMSevenTeV{\ensuremath{ 22.10 \pm 0.50\text{ fb}}}
\newcommand\PhaseSpaceXsecTheoryMMEESevenTeV{\ensuremath{ 22.10 \pm 0.50\text{ fb}}}
\newcommand\PhaseSpaceXsecTheoryMMMMSevenTeV{\ensuremath{ 22.89 \pm 0.51\text{ fb}}}
\newcommand\PhaseSpaceXsecTheorySameSevenTeV{\ensuremath{ 45.78 \pm 1.10\text{ fb}}}
\newcommand\PhaseSpaceXsecTheoryMixSevenTeV{\ensuremath{ 44.19 \pm 1.04\text{ fb}}}
\newcommand\PhaseSpaceXsecTheorySevenTeV{\ensuremath{ 89.97 \pm 2.06\text{ fb}}}
\newcommand\PhaseSpaceXsecTheoryEEEEEightTeV{\ensuremath{ 26.68 \pm 0.66\text{ fb}}}
\newcommand\PhaseSpaceXsecTheoryEEMMEightTeV{\ensuremath{ 25.75 \pm 0.64\text{ fb}}}
\newcommand\PhaseSpaceXsecTheoryMMEEEightTeV{\ensuremath{ 25.75 \pm 0.64\text{ fb}}}
\newcommand\PhaseSpaceXsecTheoryMMMMEightTeV{\ensuremath{ 26.68 \pm 0.66\text{ fb}}}
\newcommand\PhaseSpaceXsecTheorySameEightTeV{\ensuremath{ 53.35 \pm 1.24\text{ fb}}}
\newcommand\PhaseSpaceXsecTheoryMixEightTeV{\ensuremath{ 51.49 \pm 1.26\text{ fb}}}
\newcommand\PhaseSpaceXsecTheoryEightTeV{\ensuremath{ 104.84 \pm 2.50\text{ fb}}}

\newcommand\AltObsBranchingSevenTeV{\ensuremath{ \left( 3.61 \pm 0.83\text{ (stat)} \pm 0.18\text{ (syst)} \right) \times 10^{-6}}}
\newcommand\AltObsBranchingEightTeV{\ensuremath{ \left( 4.49 \pm 0.37\text{ (stat)} \pm 0.15\text{ (syst)} \right) \times 10^{-6}}}
\newcommand\AltObsBranching{\ensuremath{ \left( 4.31 \pm 0.34\text{ (stat)} \pm 0.17\text{ (syst)} \right) \times 10^{-6}}}
\newcommand\ObsBranchingSevenTeV{\ensuremath{ \left( 2.67 \pm 0.62\text{ (stat)} \pm 0.14\text{ (syst)} \right) \times 10^{-6}}}
\newcommand\ObsBranchingEightTeV{\ensuremath{ \left( 3.33 \pm 0.27\text{ (stat)} \pm 0.13\text{ (syst)} \right) \times 10^{-6}}}
\newcommand\ObsBranching{\ensuremath{ \left( 3.20 \pm 0.25\text{ (stat)} \pm 0.13\text{ (syst)} \right) \times 10^{-6}}}

\newcommand\LooseObsMMMMEightTeV{\ensuremath{ 168}}
\newcommand\LooseObsEEMMEightTeV{\ensuremath{ 102}}
\newcommand\LooseObsMMEEEightTeV{\ensuremath{ 28}}
\newcommand\LooseObsEEEEEightTeV{\ensuremath{ 23}}
\newcommand\LooseExpZjetMMMMEightTeV{\ensuremath{ 0.30 \pm 0.18}}
\newcommand\LooseExpZjetEEMMEightTeV{\ensuremath{ 0.22 \pm 0.11}}
\newcommand\LooseExpZjetMMEEEightTeV{\ensuremath{ 0.02 \pm 0.01}}
\newcommand\LooseExpZjetEEEEEightTeV{\ensuremath{ 0.02 \pm 0.01}}
\newcommand\LooseExpTtbarMMMMEightTeV{\ensuremath{ 0.33 \pm 0.33}}
\newcommand\LooseExpTtbarEEMMEightTeV{\ensuremath{ 0.08 \pm 0.08}}
\newcommand\LooseExpTtbarMMEEEightTeV{\ensuremath{ 0.00 \pm 0.00}}
\newcommand\LooseExpTtbarEEEEEightTeV{\ensuremath{ 0.08 \pm 0.08}}

\newcommand\FitMeanMCEEEEEightTeV{\ensuremath{ 89.67 \pm 0.09\text{ GeV}}}
\newcommand\FitMeanMCEEMMEightTeV{\ensuremath{ 90.01 \pm 0.04\text{ GeV}}}
\newcommand\FitMeanMCMMEEEightTeV{\ensuremath{ 90.53 \pm 0.08\text{ GeV}}}
\newcommand\FitMeanMCMMMMEightTeV{\ensuremath{ 90.73 \pm 0.03\text{ GeV}}}
\newcommand\FitMeanDataEEEEEightTeV{\ensuremath{ 89.56 \pm 0.69\text{ GeV}}}
\newcommand\FitMeanDataEEMMEightTeV{\ensuremath{ 89.44 \pm 0.33\text{ GeV}}}
\newcommand\FitMeanDataMMEEEightTeV{\ensuremath{ 89.78 \pm 0.65\text{ GeV}}}
\newcommand\FitMeanDataMMMMEightTeV{\ensuremath{ 90.63 \pm 0.29\text{ GeV}}}
\newcommand\FitRMSMCEEEEEightTeV{\ensuremath{ 3.84 \pm 0.06\text{ GeV}}}
\newcommand\FitRMSMCEEMMEightTeV{\ensuremath{ 3.73 \pm 0.03\text{ GeV}}}
\newcommand\FitRMSMCMMEEEightTeV{\ensuremath{ 3.72 \pm 0.06\text{ GeV}}}
\newcommand\FitRMSMCMMMMEightTeV{\ensuremath{ 3.48 \pm 0.02\text{ GeV}}}
\newcommand\FitRMSDataEEEEEightTeV{\ensuremath{ 3.31 \pm 0.49\text{ GeV}}}
\newcommand\FitRMSDataEEMMEightTeV{\ensuremath{ 3.36 \pm 0.24\text{ GeV}}}
\newcommand\FitRMSDataMMEEEightTeV{\ensuremath{ 3.42 \pm 0.46\text{ GeV}}}
\newcommand\FitRMSDataMMMMEightTeV{\ensuremath{ 3.75 \pm 0.20\text{ GeV}}}
\newcommand\FitMfourlMCEEEEEightTeV{\ensuremath{ 89.67 \pm 0.09\text{ GeV}}}
\newcommand\FitMfourlMCEEMMEightTeV{\ensuremath{ 90.03 \pm 0.04\text{ GeV}}}
\newcommand\FitMfourlMCMMEEEightTeV{\ensuremath{ 90.66 \pm 0.07\text{ GeV}}}
\newcommand\FitMfourlMCMMMMEightTeV{\ensuremath{ 90.87 \pm 0.03\text{ GeV}}}
\newcommand\FitMfourlDataEEEEEightTeV{\ensuremath{ 89.93 \pm 0.66\text{ GeV}}}
\newcommand\FitMfourlDataEEMMEightTeV{\ensuremath{ 89.52 \pm 0.34\text{ GeV}}}
\newcommand\FitMfourlDataMMEEEightTeV{\ensuremath{ 89.43 \pm 0.70\text{ GeV}}}
\newcommand\FitMfourlDataMMMMEightTeV{\ensuremath{ 90.59 \pm 0.30\text{ GeV}}}
\newcommand\FitFwhmMCEEEEEightTeV{\ensuremath{ 7.73 \pm 0.34\text{ GeV}}}
\newcommand\FitFwhmMCEEMMEightTeV{\ensuremath{ 7.04 \pm 0.16\text{ GeV}}}
\newcommand\FitFwhmMCMMEEEightTeV{\ensuremath{ 6.94 \pm 0.24\text{ GeV}}}
\newcommand\FitFwhmMCMMMMEightTeV{\ensuremath{ 5.14 \pm 0.10\text{ GeV}}}
\newcommand\FitFwhmDataEEEEEightTeV{\ensuremath{ 5.54 \pm 1.50\text{ GeV}}}
\newcommand\FitFwhmDataEEMMEightTeV{\ensuremath{ 5.85 \pm 0.80\text{ GeV}}}
\newcommand\FitFwhmDataMMEEEightTeV{\ensuremath{ 6.44 \pm 1.78\text{ GeV}}}
\newcommand\FitFwhmDataMMMMEightTeV{\ensuremath{ 6.29 \pm 0.75\text{ GeV}}}
\newcommand\FitWidFracMCEEEEEightTeV{\ensuremath{ 0.62 \pm 0.10}}
\newcommand\FitWidFracMCEEMMEightTeV{\ensuremath{ 0.67 \pm 0.05}}
\newcommand\FitWidFracMCMMEEEightTeV{\ensuremath{ 0.67 \pm 0.07}}
\newcommand\FitWidFracMCMMMMEightTeV{\ensuremath{ 0.87 \pm 0.03}}
\newcommand\FitFiveGeVMfourlMCEEEEEightTeV{\ensuremath{ 89.60 \pm 0.12\text{ GeV}}}
\newcommand\FitFiveGeVMfourlMCEEMMEightTeV{\ensuremath{ 90.16 \pm 0.06\text{ GeV}}}
\newcommand\FitFiveGeVMfourlMCMMEEEightTeV{\ensuremath{ 90.63 \pm 0.10\text{ GeV}}}
\newcommand\FitFiveGeVMfourlMCMMMMEightTeV{\ensuremath{ 90.90 \pm 0.04\text{ GeV}}}
\newcommand\FitFiveGeVMfourlDataEEEEEightTeV{\ensuremath{ 90.19 \pm 0.46\text{ GeV}}}
\newcommand\FitFiveGeVMfourlDataEEMMEightTeV{\ensuremath{ 89.65 \pm 0.57\text{ GeV}}}
\newcommand\FitFiveGeVMfourlDataMMEEEightTeV{\ensuremath{ 89.04 \pm 0.76\text{ GeV}}}
\newcommand\FitFiveGeVMfourlDataMMMMEightTeV{\ensuremath{ 90.49 \pm 0.42\text{ GeV}}}
\newcommand\FitFiveGeVFwhmMCEEEEEightTeV{\ensuremath{ 7.70 \pm 0.53\text{ GeV}}}
\newcommand\FitFiveGeVFwhmMCEEMMEightTeV{\ensuremath{ 7.06 \pm 0.28\text{ GeV}}}
\newcommand\FitFiveGeVFwhmMCMMEEEightTeV{\ensuremath{ 7.28 \pm 0.33\text{ GeV}}}
\newcommand\FitFiveGeVFwhmMCMMMMEightTeV{\ensuremath{ 5.29 \pm 0.15\text{ GeV}}}
\newcommand\FitFiveGeVFwhmDataEEEEEightTeV{\ensuremath{ 2.96 \pm 1.10\text{ GeV}}}
\newcommand\FitFiveGeVFwhmDataEEMMEightTeV{\ensuremath{ 6.22 \pm 1.30\text{ GeV}}}
\newcommand\FitFiveGeVFwhmDataMMEEEightTeV{\ensuremath{ 5.05 \pm 1.81\text{ GeV}}}
\newcommand\FitFiveGeVFwhmDataMMMMEightTeV{\ensuremath{ 6.59 \pm 1.05\text{ GeV}}}
\newcommand\FitFiveGeVWidFracMCEEEEEightTeV{\ensuremath{ 0.81 \pm 0.14}}
\newcommand\FitFiveGeVWidFracMCEEMMEightTeV{\ensuremath{ 0.80 \pm 0.08}}
\newcommand\FitFiveGeVWidFracMCMMEEEightTeV{\ensuremath{ 0.66 \pm 0.09}}
\newcommand\FitFiveGeVWidFracMCMMMMEightTeV{\ensuremath{ 0.85 \pm 0.05}}

\newcommand\FitDiffMMMMEightTeV{\ensuremath{ 0.28 \pm 0.30\text{ GeV}}}
\newcommand\FitDiffEEMMEightTeV{\ensuremath{ 0.51 \pm 0.34\text{ GeV}}}

\newcommand\TChanTheorySameSevenTeV{\ensuremath{ 1.55 \pm 0.04\text{ fb}}}
\newcommand\TChanTheoryMixSevenTeV{\ensuremath{ 1.73 \pm 0.04\text{ fb}}}
\newcommand\TChanTheorySevenTeV{\ensuremath{ 3.28 \pm 0.08\text{ fb}}}
\newcommand\TChanTheorySameEightTeV{\ensuremath{ 1.79 \pm 0.04\text{ fb}}}
\newcommand\TChanTheoryMixEightTeV{\ensuremath{ 2.01 \pm 0.05\text{ fb}}}
\newcommand\TChanTheoryEightTeV{\ensuremath{ 3.80 \pm 0.09\text{ fb}}}
\newcommand\AltTChanFracSame{\ensuremath{ \left( 4.04 \pm 0.02 \right)\%}}
\newcommand\AltTChanFracDiff{\ensuremath{ \left( 4.52 \pm 0.02 \right)\%}}
\newcommand\AltTChanFracSameSevenTeV{\ensuremath{ \left( 4.02 \pm 0.02 \right)\%}}
\newcommand\AltTChanFracDiffSevenTeV{\ensuremath{ \left( 4.53 \pm 0.02 \right)\%}}
\newcommand\AltTChanFracSameEightTeV{\ensuremath{ \left( 4.05 \pm 0.02 \right)\%}}
\newcommand\AltTChanFracDiffEightTeV{\ensuremath{ \left( 4.50 \pm 0.02 \right)\%}}
\newcommand\TChanFracSame{\ensuremath{ \left( 3.35 \pm 0.02 \right)\%}}
\newcommand\TChanFracDiff{\ensuremath{ \left( 3.90 \pm 0.02 \right)\%}}
\newcommand\TChanFracSameSevenTeV{\ensuremath{ \left( 3.39 \pm 0.02 \right)\%}}
\newcommand\TChanFracDiffSevenTeV{\ensuremath{ \left( 3.93 \pm 0.02 \right)\%}}
\newcommand\TChanFracSameEightTeV{\ensuremath{ \left( 3.35 \pm 0.02 \right)\%}}
\newcommand\TChanFracDiffEightTeV{\ensuremath{ \left( 3.90 \pm 0.02 \right)\%}}

\newcommand\BkgAeeeeEESRSevenTeV{\ensuremath{ 0.11 \pm 0.01 \pm 0.04 \pm 0}}
\newcommand\BkgAeemmEESRSevenTeV{\ensuremath{ 0.10 \pm 0.01 \pm 0.04 \pm 0}}
\newcommand\BkgAmmeeEESRSevenTeV{\ensuremath{ 0.04 \pm 0.00 \pm 0.02 \pm 0}}
\newcommand\BkgAmmmmEESRSevenTeV{\ensuremath{ 0}}
\newcommand\BkgAeeeeMMSRSevenTeV{\ensuremath{ 0}}
\newcommand\BkgAeemmMMSRSevenTeV{\ensuremath{ 0.05 \pm 0.03 \pm 0 \pm 0.01}}
\newcommand\BkgAmmeeMMSRSevenTeV{\ensuremath{ 0.01 \pm 0.01 \pm 0 \pm 0.00}}
\newcommand\BkgAmmmmMMSRSevenTeV{\ensuremath{ 0.05 \pm 0.03 \pm 0 \pm 0.03}}
\newcommand\BkgAeeeeEMSRSevenTeV{\ensuremath{ 0}}
\newcommand\BkgAeemmEMSRSevenTeV{\ensuremath{ 0.01 \pm 0.00 \pm 0.04 \pm 0.00}}
\newcommand\BkgAmmeeEMSRSevenTeV{\ensuremath{ 0.01 \pm 0.00 \pm 0.01 \pm 0.00}}
\newcommand\BkgAmmmmEMSRSevenTeV{\ensuremath{ 0}}
\newcommand\BkgAeeeeTotalSRSevenTeV{\ensuremath{ 0.11 \pm 0.05}}
\newcommand\BkgAeemmTotalSRSevenTeV{\ensuremath{ 0.16 \pm 0.09}}
\newcommand\BkgAmmeeTotalSRSevenTeV{\ensuremath{ 0.06 \pm 0.03}}
\newcommand\BkgAmmmmTotalSRSevenTeV{\ensuremath{ 0.05 \pm 0.04}}
\newcommand\BkgATotalTotalSRSevenTeV{\ensuremath{ 0.38 \pm 0.14}}
\newcommand\BkgAeeeeEESREightTeV{\ensuremath{ 0.10 \pm 0.00 \pm 0.01 \pm 0}}
\newcommand\BkgAeemmEESREightTeV{\ensuremath{ 0.10 \pm 0.00 \pm 0.02 \pm 0}}
\newcommand\BkgAmmeeEESREightTeV{\ensuremath{ 0.06 \pm 0.00 \pm 0.01 \pm 0}}
\newcommand\BkgAmmmmEESREightTeV{\ensuremath{ 0}}
\newcommand\BkgAeeeeMMSREightTeV{\ensuremath{ 0}}
\newcommand\BkgAeemmMMSREightTeV{\ensuremath{ 0.06 \pm 4.03 \pm 0 \pm 0.01}}
\newcommand\BkgAmmeeMMSREightTeV{\ensuremath{ 0.00 \pm 0.00 \pm 0 \pm 0.00}}
\newcommand\BkgAmmmmMMSREightTeV{\ensuremath{ 0.11 \pm 0.03 \pm 0 \pm 0.03}}
\newcommand\BkgAeeeeEMSREightTeV{\ensuremath{ 0}}
\newcommand\BkgAeemmEMSREightTeV{\ensuremath{ 0.04 \pm 0.00 \pm 0.03 \pm 0.01}}
\newcommand\BkgAmmeeEMSREightTeV{\ensuremath{ 0.02 \pm 0.00 \pm 0.01 \pm 0.00}}
\newcommand\BkgAmmmmEMSREightTeV{\ensuremath{ 0}}
\newcommand\BkgAeeeeTotalSREightTeV{\ensuremath{ 0.10 \pm 0.01}}
\newcommand\BkgAeemmTotalSREightTeV{\ensuremath{ 0.24 \pm 0.05}}
\newcommand\BkgAmmeeTotalSREightTeV{\ensuremath{ 0.08 \pm 0.02}}
\newcommand\BkgAmmmmTotalSREightTeV{\ensuremath{ 0.11 \pm 0.05}}
\newcommand\BkgATotalTotalSREightTeV{\ensuremath{ 0.49 \pm 0.10}}

\newcommand\ExpectedTotalEEEESevenTeV{\ensuremath{ 1.8 \pm 0.3}}
\newcommand\ExpectedTotalEEMMSevenTeV{\ensuremath{ 8.0 \pm 0.4}}
\newcommand\ExpectedTotalMMEESevenTeV{\ensuremath{ 3.3 \pm 0.3}}
\newcommand\ExpectedTotalMMMMSevenTeV{\ensuremath{ 11.3 \pm 0.5}}
\newcommand\ExpectedTotalAllSevenTeV{\ensuremath{ 24.4 \pm 1.2}}
\newcommand\ExpectedTotalEEEEEightTeV{\ensuremath{  79.58 \pm 0.49 \pm 3.71}}
\newcommand\ExpectedTotalEEMMEightTeV{\ensuremath{ 103.91 \pm 0.58 \pm 2.31}}
\newcommand\ExpectedTotalMMEEEightTeV{\ensuremath{ 101.27 \pm 0.91 \pm 2.93}}
\newcommand\ExpectedTotalMMMMEightTeV{\ensuremath{ 150.17 \pm 0.70 \pm 2.78}}
\newcommand\ExpectedTotalAllEightTeV{\ensuremath{  435.02 \pm 1.34 \pm 9.32}}

\newcommand\ExpectedTotalNNLOEEEEEightTeV{\ensuremath{  87.00 \pm 0.51 \pm 4.07}}
\newcommand\ExpectedTotalNNLOEEMMEightTeV{\ensuremath{ 111.44 \pm 0.61 \pm 2.52}}
\newcommand\ExpectedTotalNNLOMMEEEightTeV{\ensuremath{ 110.66 \pm 0.93 \pm 3.22}}
\newcommand\ExpectedTotalNNLOMMMMEightTeV{\ensuremath{ 162.06 \pm 0.72 \pm 3.00}}
\newcommand\ExpectedTotalNNLOAllEightTeV{\ensuremath{  470.96 \pm 1.39 \pm 10.16}}


\newcommand\ExpectedAllTotal{\ensuremath{ 169 \pm 12}}
\newcommand\AltExpectedBranching{\ensuremath{ \left( 4.50 \pm 0.01 \right) \times 10^{-6}}}
\newcommand\ExpectedBranching{\ensuremath{ \left( 3.33 \pm 0.01 \right) \times 10^{-6}}}

\newcommand\CMSObsBranching{\ensuremath{ \left( 4.2^{+0.9}_{-0.8}\text{ (stat)} \pm 0.2\text{ (syst)} \right) \times 10^{-6}}}
\newcommand\CMSExpBranching{\ensuremath{ 4.45 \times 10^{-6}}}
\newcommand\ExpDDLLJJEEEE{\ensuremath{ 1.68 \pm 0.01}}
\newcommand\ExpDDLLJJEEMM{\ensuremath{ 1.03 \pm 0.09}}
\newcommand\ExpDDLLJJMMEE{\ensuremath{ 2.60 \pm 0.02}}
\newcommand\ExpDDLLJJMMMM{\ensuremath{ 0.86 \pm 0.11}}
\newcommand\ExpDDLLJJAll{\ensuremath{  6.17 \pm 0.14}}

\newcommand\ExpDDLLLJEEEE{\ensuremath{ 3.72 \pm 0.16}}
\newcommand\ExpDDLLLJEEMM{\ensuremath{ 3.88 \pm 0.52}}
\newcommand\ExpDDLLLJMMEE{\ensuremath{ 5.45 \pm 0.24}}
\newcommand\ExpDDLLLJMMMM{\ensuremath{ 8.27 \pm 1.75}}
\newcommand\ExpDDLLLJAll{\ensuremath{ 21.34 \pm 1.85}}

\newcommand\ExpDDEEEE{\ensuremath{  2.04 \pm 0.16 \pm 0.34}}
\newcommand\ExpDDEEMM{\ensuremath{  2.85 \pm 0.52 \pm 0.13}}
\newcommand\ExpDDMMEE{\ensuremath{  2.86 \pm 0.24 \pm 0.41}}
\newcommand\ExpDDMMMM{\ensuremath{  7.41 \pm 1.75 \pm 2.27}}
\newcommand\ExpDDAll{\ensuremath{  15.16 \pm 1.86 \pm 2.23}}

\newcommand\ExpZgammaMCAllEightTeV{\ensuremath{      2.55 \pm       1.00}}
\newcommand\ExpVVVMCAllEightTeV{\ensuremath{      1.08 \pm       0.03}}
\newcommand\ExpTtbarMCAllEightTeV{\ensuremath{      2.13 \pm       0.18}}
\newcommand\ExpGGHMCAllEightTeV{\ensuremath{     13.69 \pm       0.09}}
\newcommand\ExpVHMCAllEightTeV{\ensuremath{      0.84 \pm       0.01}}
\newcommand\ExpTtHMCAllEightTeV{\ensuremath{      0.10 \pm       0.00}}
\newcommand\ExpVBFHMCAllEightTeV{\ensuremath{      4.56 \pm       0.02}}
\newcommand\ExpDPIMCAllEightTeV{\ensuremath{      0.39 \pm       0.00}}
\newcommand\ExpWZMCAllEightTeV{\ensuremath{      1.55 \pm       0.26}}
\newcommand\ExpTtbarZMCAllEightTeV{\ensuremath{      2.96 \pm       0.12}}
\newcommand\ExpTtbarWMCAllEightTeV{\ensuremath{      0.03 \pm       0.02}}
\newcommand\ExpTZMCAllEightTeV{\ensuremath{      0.60 \pm       0.04}}
\newcommand\ExpZjetMCAllEightTeV{\ensuremath{      0.80 \pm       0.60}}
\newcommand\ExpZbbMCAllEightTeV{\ensuremath{      6.90 \pm       0.23}}
\newcommand\ExpZHZZllnnMCAllEightTeV{\ensuremath{      0.27 \pm       0.02}}
\newcommand\ExpZgammaMCEEEEEightTeV{\ensuremath{      1.28 \pm       0.77}}
\newcommand\ExpVVVMCEEEEEightTeV{\ensuremath{      0.22 \pm       0.01}}
\newcommand\ExpTtbarMCEEEEEightTeV{\ensuremath{      0.38 \pm       0.08}}
\newcommand\ExpGGHMCEEEEEightTeV{\ensuremath{      2.31 \pm       0.04}}
\newcommand\ExpVHMCEEEEEightTeV{\ensuremath{      0.15 \pm       0.00}}
\newcommand\ExpTtHMCEEEEEightTeV{\ensuremath{      0.02 \pm       0.00}}
\newcommand\ExpVBFHMCEEEEEightTeV{\ensuremath{      0.89 \pm       0.01}}
\newcommand\ExpDPIMCEEEEEightTeV{\ensuremath{      0.06 \pm       0.00}}
\newcommand\ExpWZMCEEEEEightTeV{\ensuremath{      0.31 \pm       0.11}}
\newcommand\ExpTtbarZMCEEEEEightTeV{\ensuremath{      0.51 \pm       0.05}}
\newcommand\ExpTtbarWMCEEEEEightTeV{\ensuremath{      0.00 \pm       0.00}}
\newcommand\ExpTZMCEEEEEightTeV{\ensuremath{      0.11 \pm       0.01}}
\newcommand\ExpZjetMCEEEEEightTeV{\ensuremath{      0.00 \pm       0.00}}
\newcommand\ExpZbbMCEEEEEightTeV{\ensuremath{      1.01 \pm       0.12}}
\newcommand\ExpZHZZllnnMCEEEEEightTeV{\ensuremath{      0.05 \pm       0.01}}
\newcommand\ExpZgammaMCEEMMEightTeV{\ensuremath{      0.00 \pm       0.00}}
\newcommand\ExpVVVMCEEMMEightTeV{\ensuremath{      0.26 \pm       0.01}}
\newcommand\ExpTtbarMCEEMMEightTeV{\ensuremath{      0.62 \pm       0.10}}
\newcommand\ExpGGHMCEEMMEightTeV{\ensuremath{      3.66 \pm       0.05}}
\newcommand\ExpVHMCEEMMEightTeV{\ensuremath{      0.21 \pm       0.00}}
\newcommand\ExpTtHMCEEMMEightTeV{\ensuremath{      0.02 \pm       0.00}}
\newcommand\ExpVBFHMCEEMMEightTeV{\ensuremath{      1.15 \pm       0.01}}
\newcommand\ExpDPIMCEEMMEightTeV{\ensuremath{      0.10 \pm       0.00}}
\newcommand\ExpWZMCEEMMEightTeV{\ensuremath{      0.44 \pm       0.15}}
\newcommand\ExpTtbarZMCEEMMEightTeV{\ensuremath{      0.78 \pm       0.06}}
\newcommand\ExpTtbarWMCEEMMEightTeV{\ensuremath{      0.02 \pm       0.01}}
\newcommand\ExpTZMCEEMMEightTeV{\ensuremath{      0.11 \pm       0.01}}
\newcommand\ExpZjetMCEEMMEightTeV{\ensuremath{      0.00 \pm       0.00}}
\newcommand\ExpZbbMCEEMMEightTeV{\ensuremath{      2.22 \pm       0.14}}
\newcommand\ExpZHZZllnnMCEEMMEightTeV{\ensuremath{      0.06 \pm       0.01}}
\newcommand\ExpZgammaMCMMEEEightTeV{\ensuremath{      1.26 \pm       0.63}}
\newcommand\ExpVVVMCMMEEEightTeV{\ensuremath{      0.25 \pm       0.01}}
\newcommand\ExpTtbarMCMMEEEightTeV{\ensuremath{      0.55 \pm       0.09}}
\newcommand\ExpGGHMCMMEEEightTeV{\ensuremath{      2.78 \pm       0.04}}
\newcommand\ExpVHMCMMEEEightTeV{\ensuremath{      0.18 \pm       0.00}}
\newcommand\ExpTtHMCMMEEEightTeV{\ensuremath{      0.02 \pm       0.00}}
\newcommand\ExpVBFHMCMMEEEightTeV{\ensuremath{      1.01 \pm       0.01}}
\newcommand\ExpDPIMCMMEEEightTeV{\ensuremath{      0.09 \pm       0.00}}
\newcommand\ExpWZMCMMEEEightTeV{\ensuremath{      0.50 \pm       0.14}}
\newcommand\ExpTtbarZMCMMEEEightTeV{\ensuremath{      0.70 \pm       0.06}}
\newcommand\ExpTtbarWMCMMEEEightTeV{\ensuremath{      0.01 \pm       0.01}}
\newcommand\ExpTZMCMMEEEightTeV{\ensuremath{      0.15 \pm       0.02}}
\newcommand\ExpZjetMCMMEEEightTeV{\ensuremath{      0.54 \pm       0.54}}
\newcommand\ExpZbbMCMMEEEightTeV{\ensuremath{      1.12 \pm       0.12}}
\newcommand\ExpZHZZllnnMCMMEEEightTeV{\ensuremath{      0.07 \pm       0.01}}
\newcommand\ExpZgammaMCMMMMEightTeV{\ensuremath{      0.00 \pm       0.00}}
\newcommand\ExpVVVMCMMMMEightTeV{\ensuremath{      0.35 \pm       0.02}}
\newcommand\ExpTtbarMCMMMMEightTeV{\ensuremath{      0.58 \pm       0.10}}
\newcommand\ExpGGHMCMMMMEightTeV{\ensuremath{      4.94 \pm       0.06}}
\newcommand\ExpVHMCMMMMEightTeV{\ensuremath{      0.30 \pm       0.00}}
\newcommand\ExpTtHMCMMMMEightTeV{\ensuremath{      0.03 \pm       0.00}}
\newcommand\ExpVBFHMCMMMMEightTeV{\ensuremath{      1.50 \pm       0.01}}
\newcommand\ExpDPIMCMMMMEightTeV{\ensuremath{      0.14 \pm       0.00}}
\newcommand\ExpWZMCMMMMEightTeV{\ensuremath{      0.30 \pm       0.11}}
\newcommand\ExpTtbarZMCMMMMEightTeV{\ensuremath{      0.96 \pm       0.07}}
\newcommand\ExpTtbarWMCMMMMEightTeV{\ensuremath{      0.00 \pm       0.00}}
\newcommand\ExpTZMCMMMMEightTeV{\ensuremath{      0.23 \pm       0.03}}
\newcommand\ExpZjetMCMMMMEightTeV{\ensuremath{      0.26 \pm       0.26}}
\newcommand\ExpZbbMCMMMMEightTeV{\ensuremath{      2.54 \pm       0.09}}
\newcommand\ExpZHZZllnnMCMMMMEightTeV{\ensuremath{      0.09 \pm       0.01}}
\newcommand\ExpZHWWlnlnMCAllEightTeV{\ensuremath{      1.27 \pm       0.12}}
\newcommand\ExpZHWWlnlnMCEEEEEightTeV{\ensuremath{      0.30 \pm       0.06}}
\newcommand\ExpZHWWlnlnMCEEMMEightTeV{\ensuremath{      0.35 \pm       0.06}}
\newcommand\ExpZHWWlnlnMCMMEEEightTeV{\ensuremath{      0.25 \pm       0.06}}
\newcommand\ExpZHWWlnlnMCMMMMEightTeV{\ensuremath{      0.37 \pm       0.07}}
\newcommand\ExpggTauMCAllEightTeV{\ensuremath{      6.54 \pm       0.14}}
\newcommand\ExpggTauMCEEEEEightTeV{\ensuremath{      1.28 \pm       0.06 \pm 0}}
\newcommand\ExpggTauMCEEMMEightTeV{\ensuremath{      1.35 \pm       0.06}}
\newcommand\ExpggTauMCMMEEEightTeV{\ensuremath{      1.73 \pm       0.07}}
\newcommand\ExpggTauMCMMMMEightTeV{\ensuremath{      2.18 \pm       0.09}}
\newcommand\ExpqqTauMCAllEightTeV{\ensuremath{      5.78 \pm       0.11}}
\newcommand\ExpqqTauMCEEEEEightTeV{\ensuremath{      1.17 \pm       0.05}}
\newcommand\ExpqqTauMCEEMMEightTeV{\ensuremath{      1.08 \pm       0.05}}
\newcommand\ExpqqTauMCMMEEEightTeV{\ensuremath{      1.62 \pm       0.06}}
\newcommand\ExpqqTauMCMMMMEightTeV{\ensuremath{      1.92 \pm       0.07}}
\newcommand\ExpggHonTauMCAllEightTeV{\ensuremath{      0.33 \pm       0.09}}
\newcommand\ExpggHonTauMCEEEEEightTeV{\ensuremath{      0.03 \pm       0.04}}
\newcommand\ExpggHonTauMCEEMMEightTeV{\ensuremath{      0.10 \pm       0.05}}
\newcommand\ExpggHonTauMCMMEEEightTeV{\ensuremath{      0.03 \pm       0.04}}
\newcommand\ExpggHonTauMCMMMMEightTeV{\ensuremath{      0.17 \pm       0.06}}
\newcommand\ExpVBFHonTauMCAllEightTeV{\ensuremath{      0.023 \pm       0.010}}
\newcommand\ExpVBFHonTauMCEEEEEightTeV{\ensuremath{      0.006 \pm       0.005}}
\newcommand\ExpVBFHonTauMCEEMMEightTeV{\ensuremath{      0.002 \pm       0.005}}
\newcommand\ExpVBFHonTauMCMMEEEightTeV{\ensuremath{      0.003 \pm       0.005}}
\newcommand\ExpVBFHonTauMCMMMMEightTeV{\ensuremath{      0.012 \pm       0.007}}


\newcommand\ExpZHZZllqqMCAllEightTeV{\ensuremath{      0.50 \pm       0.03}}
\newcommand\ExpZHZZllqqMCEEEEEightTeV{\ensuremath{      0.11 \pm       0.01}}
\newcommand\ExpZHZZllqqMCEEMMEightTeV{\ensuremath{      0.13 \pm       0.02}}
\newcommand\ExpZHZZllqqMCMMEEEightTeV{\ensuremath{      0.09 \pm       0.01}}
\newcommand\ExpZHZZllqqMCMMMMEightTeV{\ensuremath{      0.16 \pm       0.02}}

